Enhancing Efficiency of Safe Reinforcement Learning via Sample Manipulation

Safe reinforcement learning (RL) is crucial for deploying RL agents in real-world applications, as it aims to maximize long-term rewards while satisfying safety constraints. However, safe RL often suffers from sample inefficiency, requiring extensive interactions with the environment to learn a safe policy. We propose Efficient Safe Policy Optimization (ESPO), a novel approach that enhances the efficiency of safe RL through sample manipulation. ESPO employs an optimization framework with three modes: maximizing rewards, minimizing costs, and balancing the trade-off between the two. By dynamically adjusting the sampling process based on the observed conflict between reward and safety gradients, ESPO theoretically guarantees convergence, optimization stability, and improved sample complexity bounds. Experiments on the Safety-MuJoCo and Omnisafe benchmarks demonstrate that ESPO significantly outperforms existing primal-based and primal-dual-based baselines in terms of reward maximization and constraint satisfaction. Moreover, ESPO achieves substantial gains in sample efficiency, requiring 25--29% fewer samples than baselines, and reduces training time by 21--38%.

==> files/sources/theory-part.tex <==

\section{Advantages of ESPO: theoretical analysis}
In this section, to further evaluate the advantages of our proposed algorithm ESPO, we provide the convergence rate and provable stability and sample complexity advancement compared to the baseline CRPO. 

\paragraph{Tabular setting with softmax policy class.}
We focus on a fundamental tabular setting with finite state and action space. We consider the class of policy with the softmax parameterization which is complete including all stochastic policies. Specifically, a policy $\pi_w$ associated with some parameter $w\in \mathbb{R}^{|\cS| |\cA|}$ is defined as
{\small \begin{align}
\forall(s,a)\in \cA\times \cS: \quad \pi_w(a|s)\coloneqq \frac{\exp(w(s,a))}{\sum_{a^\prime \in \cA}\exp(w(s,a^\prime))}. \label{eq:2}
\end{align}}

 
Before proceeding, we introduce some useful notations. Let $\nr$, $\nsoft$ (includes $\nsoft^{\mathsf{conf}}$ and $\nsoft^{\mathsf{no}}$) and $\nc$ denote the set of iteration indexes that our proposed \textsf{ESPO} execute in the case of \lxs{to fill refer to the algorithm later}.


\subsection{Provable convergence of ESPO}
First, we present the convergence rate of our proposed ESPO in terms of both the optimal reward and  the constraint requirement in the following theorem; the proof is given in Appendix~\ref{proof:thm:convergence}.


\begin{theorem}\label{thm:convergence}
Consider tabular setting with policy class defined in \eqref{eq:2}, and any $\delta \in (0,1)$. For Algorithm~\ref{alg:ESPO-framework-gradually}, take $K_{\text{in}}=\Theta(T^{1/\sigma}(1-\gamma)^{-2/\sigma}\log^{2/\sigma}(T^{1+2/\sigma}/\delta))$ iterations for policy evaluation in , set tolerance $\eta $ and perform the NPG update rule defined in with $\alpha $. Then, the output $\widehat{\pi}$ of Algorithm~\ref{alg:ESPO-framework-gradually} satisfies with probability at least $1-\delta$ that
	 \begin{align}
     V_r(\pi^\star) -  \mathbb{E}[V_r(\widehat{\pi})] \leq \widetilde{O}\left(\sqrt{\frac{SA}{(1-\gamma)^3T}}\right) \notag \\
   \mathbb{E}[V_c(\widehat{\pi})] - V_c(\pi^\star)  \leq \widetilde{O}\left(\sqrt{\frac{SA}{(1-\gamma)^3T}}\right).
   \end{align}
%    and
%    \begin{flalign*}
%    	\sE[J_i(w_{\text{out}})] - d_i =\mathcal{O}\left( \frac{\sqrt{\lone{\mcs}\lone{\mca}}}{(1-\gamma)^{1.5}\sqrt{T}} \right), \quad \text{for all}\quad i=1,\cdots,p,
%    \end{flalign*}
Here, the expectation is taken with respect to selecting $\widehat{\pi}$ from $\{\pi_{w_t}\}_{1\leq i \leq T}$ with certain weights.
\end{theorem}

Theorem~\ref{thm:convergence} shows that the proposed algorithm ESPO converges to a global optimal policy $\pi^\star$ in the feasible set at the rate of $\widetilde{O}\left(\sqrt{\frac{SA}{(1-\gamma)^3T}} \right)$. The constraint violation also converges to $0$ at the rate of $\widetilde{O}\left(\sqrt{\frac{SA}{(1-\gamma)^3T}}\right)$. ESPO enjoys the same convergence rate as CRPO \citep{xu2021crpo}. As the update rule of ESPO varies based on the conflict condition, deriving the results requires a tailored weighting for selecting policies from $\{\pi_{w_t}\}_{1\leq i \leq T}$.

\subsection{Advantages of the proposed method}
We will introduce two advantages of ESPO in terms of both optimization and sample efficiency.


\paragraph{Efficient optimization with reduced oscillation.}
Shown qualitatively in Figure~\ref{fig:comparison-oscillation-methods}, our proposed ESPO can significantly increase the ratio of iterations for maximizing the reward objective. In the following theorem, we provide a rigorous quantitative analysis for such advancement:
\begin{proposition}
    From any initial point $w_0\in\mathbb{R}^{|\cS||\cA|}$, by adaptively choosing the algorithm parameters in Algorithm~\ref{alg:ESPO-framework-gradually}, if there exist iteration $t_{\mathsf{in}}<T$ such that $t\in \nr \cup \nsoft$, one has
    \begin{align}
    &\forall t_{\mathsf{in}} \leq t \leq T: \quad t \in \nr \cup \nsoft \notag \\
    &|\nr| + |\nsoft| \geq \cB_r^{\mathsf{CRPO}}
    \end{align}
\end{proposition}

In words, the above theorem indicates two facts. First, as long as ESPO (Algorithm~\ref{alg:ESPO-framework-gradually} enters the region that the constraint  violated is at most $\eta$, it will never go out. This reduces the oscillation in and out of the constraint feasible set. It leads to the second fact that the proposed ESPO will have more iterations involving maximizing the reward objective compared to CRPO, accelerating the convergence towards the global optimal policy.



\paragraph{Sample efficiency with adaptive batch size.}
Besides the efficient optimization of ESPO, the following theorem presents the sample efficiency of ESPO.
\begin{proposition}
    Consider any accuracy level $ 0 \leq \varepsilon \leq \frac{1}{1-\gamma}$, to meet the following goal of performance gap
    \begin{align}
        V_r(\pi^\star) -  \mathbb{E}[V_r(\widehat{\pi})] \leq \varepsilon,
    \end{align}
    Algorithm~\ref{alg:ESPO-framework-gradually} need less total number of samples than Algorithm~\ref{alg:ESPO-framework-gradually} without the adaptive sample size adjustment in line.
\end{proposition}

The results show that to meet the certain accuracy requirement, the adaptive sampling approach leads to more sample efficiency algorithm by using the conflicting between the gradient associated with reward and cost as the metric. It indicates that we should have a more accurate update direction when the reward and cost objective has conflict of interest.


